Exploring In-Context Learning of Textless Speech Language Model for Speech Classification Tasks

Ever since the development of GPT-3 in the natural language processing (NLP) field, in-context learning (ICL) has played an essential role in utilizing large language models (LLMs). By presenting the LM utterance-label demonstrations at the input, the LM can accomplish few-shot learning without relying on gradient descent or requiring explicit modification of its parameters. This enables the LM to perform various downstream tasks in a black-box manner. Despite the success of ICL in NLP, little work is exploring the possibility of ICL in speech processing. This study is the first work exploring ICL for speech classification tasks with textless speech LM. We first show that the current speech LM lacks the ICL capability. We then perform warmup training on the speech LM, equipping the LM with demonstration learning capability. This paper explores and proposes the first speech LM capable of performing unseen classification tasks in an ICL manner.

==> pic/data.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.96\textwidth]{pic/data2.png}
    \caption{This diagram illustrates the data structure associated with in-context learning.}
    \label{fig:enter-label}
\end{figure*}

==> pic/prompt_length_pic.tex <==
% \begin{figure}
%     \centering
% \includegraphics[width=0.48\textwidth]{pic/prompt_length4.png}
%     \caption{}
%     \label{fig:prompt-length}
% \end{figure}

==> pic/structure.tex <==
\begin{figure*}
    \centering
\includegraphics[width=0.89\textwidth]{pic/Model11.png}
    \caption{The figure illustrates the in-context learning method in our work. The model predicts the label of the target utterance conditioned on demonstrations and the prompts. During the whole process, the backbone GSLM is fixed.}
    % \caption{The figure illustrates the comprehensive structure of the model implemented in our ICL method.}
    \label{fig:model-arch}
\end{figure*}

==> pic/test_process.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.48\textwidth]{pic/test_process.png}
    \caption{}
    \label{fig:test_process}
\end{figure}

==> tables/dataset_size.tex <==
% \begin{table*}[]
%     \centering
%     \begin{tabular}
%         {@{}c|ccc@{}}\toprule
%         \textbf{Dataset Size}& 10000 & 25000 & 50000 \\
%         \cmidrule{1-4}
%         Testing Dataset 1 & 40.94\% $\pm$ 1.47\% & \textbf{42.74\%} $\pm$ \textbf{1.10\%} & 36.26\% $\pm$ 1.38\% \\
%         Testing Dataset 2 & 54.14\% $\pm$ 0.80\% & 54.74\% $\pm$ 0.96\% & \textbf{75.66\%} $\pm$ \textbf{0.91\%} \\
%         Training Dataset & 82.04\% $\pm$ 0.67\% & 78.42\% $\pm$ 1.24\% & \textbf{80.16\%} $\pm$ \textbf{0.72\%}\\
%         \cmidrule{1-4}
%     \end{tabular}
%     \caption{This table provides a comparison of the impacts associated with various sizes of training datasets.}
%     \label{tab:dataset_size}
% \end{table*}
\begin{table}[]
    \centering
    \begin{tabular}
        {@{}cc>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}@{}}%\toprule
        \Xhline{2pt}
        \multicolumn{2}{c}{\textbf{Dataset Size}}& 10 k & 25 k & 50 k \\
        % \cmidrule{1-4}
        \Xhline{0.4pt}
        \multirow{3}{1.2cm}{\centering Group 1\\$\mathcal{T}_{test}$}& Arabic SC & 40.9 & \textbf{42.7} & 36.3 \\
        &ASVspoof & 51.9 & \textbf{52.5} & 52.2 \\
        &IEMOCAP & \textbf{47.7} & 47.4 & 46.9 \\
        % \cmidrule{1-4}
        \Xhline{2pt}
    \end{tabular}
    \caption{Accuracy comparison across different training dataset sizes. Model performance does not drastically change with dataset size, indicating only a sufficient amount of data is needed to learn the task, not an extensive dataset.}
    \label{tab:dataset_size}
\end{table}


==> tables/datasets.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}
%         {@{}c|c@{}}\toprule
%         Usage & Datasets\\
%         \cmidrule{1-2}
%         \multirow{2}*{Training Dataset} & SCR LT, SCR DM, SCR Google\\
%         ~ & LID voxforge, SD mustard\\
%         \cmidrule{1-2}
%         Testing Dataset 1& SCR AR \\
%         % \cmidrule{1-2}
%         % Testing Dataset 2& ER iemocap \\
%         % \cmidrule{1-2}
%         Testing Dataset 2& FSD asvspoof \\
%     \end{tabular}
%     \caption{This table shows the training and testing datasets.}
%     \label{tab:datasets}
% \end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
        \toprule
        Group & Usage & Datasets\\
        \cmidrule{1-3}
        \multirow{8}{*}{Group 1} & \multirow{5}{*}{Training Dataset} & Lithuanian SC~\cite{}\\
        & & Dysarthric Mandarin SC\\
        & & Google SC v2\\
        & & Voxforge\\
        & & MUStARD\\
        \cmidrule{2-3}
        & \multirow{3}{*}{Testing Dataset} & Arabic SC\\
        & & ASVspoof\\
        & & IEMOCAP\\
        \cmidrule{1-3}
        \multirow{8}{*}{Group 2} & \multirow{4}{*}{Training Dataset} & Lithuanian SC\\
        & & Dysarthric Mandarin SC\\
        & & Voxforge\\
        & & IEMOCAP\\
        \cmidrule{2-3}
        & \multirow{4}{*}{Testing Dataset} & Google SC v2\\
        & & Arabic SC\\
        & & MAStARD\\
        & & ASVspoof\\
        \bottomrule
    \end{tabular}
    \caption{This table shows the training and testing datasets.}
    \label{tab:datasets}
\end{table}



==> tables/fine_tuning.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}
%         {@{}c|cc@{}}\toprule
%         & Ours & Finetuning  \\
%         \cmidrule{1-3}
%         Testing Set 1  & \textbf{40.94\%} $\pm$ \textbf{1.47\%} & 30.94\% $\pm$ 2.03\% \\
%         % Testing Set 2  & \textbf{47.74\%} $\pm$ \textbf{1.82\%} & 39.24\% $\pm$ 0.79\%  \\
%         Testing Set 2  & 54.14\% $\pm$ 0.81\% & \textbf{74.20\%} $\pm$ \textbf{1.26\%} \\
%         Training Set & 82.04\% $\pm$ 0.67\% & \textbf{82.96\%} $\pm$ \textbf{1.19\%}  \\
%     \end{tabular}
%     \caption{The table presents a comparative analysis between our method, as described earlier (see Table \ref{tab:main_table}), and the outcome of fine-tuning the entire GSLM model.}
%     \label{tab:finetune_table}
% \end{table}

% % \textcolor{red}{TODO: If not use same dataset for testing, need bold?}

\begin{table}[]
    \centering
    \begin{tabular}
        {@{}cc>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{2cm}@{}}%\toprule
        \Xhline{2pt}
        \multicolumn{2}{c}{\textbf{Method}}& Ours & Finetuning\\
        % \cmidrule{1-3}
        \Xhline{0.4pt}
        \multirow{3}{1.2cm}{\centering Group 1\\$\mathcal{T}_{test}$}&Arabic SC & \textbf{40.9} & 30.9\\
        &ASVspoof & 51.9 & \textbf{74.2}\\
        &IEMOCAP & \textbf{47.7} & 39.2\\
        % \cmidrule{1-3}
        \Xhline{2pt}
    \end{tabular}
    % \caption{Performance comparison between prompt tuning (Ours) and finetuning the entire model. Prompt tuning demonstrates better overall performance on unseen tasks.}
    \caption{Accuracy comparison between prompt tuning and fine-tuning the whole model in warmup training. Fine-tuning the whole model causes instability for ICL.}
    \label{tab:finetune_table}
\end{table}


==> tables/prompt_length_analysis.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{@{}cc>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}@{}}%\toprule
    \Xhline{2pt}
    \multicolumn{2}{c}{\textbf{Prompt Length}}& 5 & 10 & 25 & 50 & 100 \\
    % \cmidrule{1-6}
    % \Xcline{}
    \Xhline{0.4pt}
    \multirow{3}{1.2cm}{\centering Group 1\\$\mathcal{T}_{test}$}& Arabic SC & \textbf{40.9} & 24.7 & 21.0 & 29.8 & 24.8\\
    & ASVspoof & 51.9 & 49.2 & \textbf{57.5} & 55.9 & 51.5\\
    & IEMOCAP & 47.7 & 47.7 & \textbf{48.5} & 46.0 & 45.4\\
    % \cmidrule{1-6}
    \Xhline{2pt}
    \end{tabular}
    \caption{Accuracy comparison across different prompt lengths. Moderate prompt lengths like 5 and 10 achieve the best overall performance, while overly long prompts can reduce performance due to overfitting.}
    \label{tab:prompt_table}
\end{table}



==> text/3_related_works.tex <==
\section{Related Works}
\label{sec:relatedworks}

% https://github.com/dongguanting/In-Context-Learning_PaperList

\subsection{In-context Learning}

In recent years, there has been a growing interest in large-language models (LLMs). 
One notable LLM is GPT-3~\cite{brown2020language}, which has introduced a new paradigm known as \emph{in-context learning (ICL)}~\cite{dong2022survey}.
ICL does not involve gradient descent and parameter updates during learning. It relies on the demonstrations to guide the model's prediction.
While some LLMs have shown the ability for ICL, a disparity persists between the LM's pre-training task and ICL. Therefore, some studies attempted to perform \emph{warmup training}~\cite{dong2022survey} to enhance the ICL capability in a supervised~\cite{min2022metaicl} or self-supervised~\cite{chen2022improving, DBLP:conf/acl/Gu0WH23} manner.
However, it is worth mentioning that these efforts have primarily concentrated on LLMs in the NLP domain. 
Despite the development of several speech-based LMs in recent years, there has been limited exploration of ICL on speech LMs.

% In speech processing, one relevant work is WavPrompt~\cite{gao2022wavprompt}. 
% It integrates an audio encoder and a text LM (specifically, GPT-2~\cite{radford2019language}). This model is then pre-trained using paired data with an automatic speech recognition (ASR) task, allowing the model to make predictions based on task demonstrations that incorporate both speech and text question-answer pairs.
% Another recent work utilizing ICL for speech processing is presented in~\cite{wang2023can}. This work uses speech-transcription pairs as demonstrations, which are then fed into Whipser~\cite{radford2023robust} for test-time adaptation in ASR.
% However, both~\cite{gao2022wavprompt} and ~\cite{wang2023can} focus on limited speech processing tasks, (Spoken Language Understanding) SLU and ASR, and utilizes models pre-trained on speech-text paired data. In contrast, our work emphasizes the use of speech LM for diverse tasks without relying on text supervision.

\subsection{Speech Language Models}
With the advancements in self-supervised speech models~\cite{mohamed2022self}, including CPC~\cite{oord2018representation}, wav2vec2.0~\cite{baevski2020wav2vec}, HuBERT~\cite{hsu2021hubert}, and w2v-BERT~\cite{chung2021w2v}, training speech LMs based on these informative representations has become promising.
Generative Spoken Language Modeling (GSLM)~\cite{lakhotia2021generative} is a pioneer work. 
GSLM proposed performing speech quantization on these speech representations to obtain discrete speech tokens. A generative LM is then trained using these speech tokens, and it has shown promising results in generating novel speech conditionally or unconditionally.

Besides GSLM, other speech LMs are also proposed with training larger models and datasets~\cite{hassid2023textually}, or incorporating speech neural codecs~\cite{zeghidour2021soundstream, défossez2022high, 10096509} to provide more informative information for language modeling~\cite{borsos2023audiolm}.
For this research, we have chosen to adopt GSLM as our backbone model because of its availability as an open-source generative speech LM. We believe that as diverse speech LMs continue to advance, the significance of ICL behavior will become increasingly evident, mirroring the observations made in the field of natural language processing (NLP)~\cite{wei2022emergent, webb2022emergent}. 

It is worth noting that VALL-E~\cite{wang2023neural, zhang2023speak} also claims to demonstrate ICL capability. However, we would like to emphasize the differences between our work and VALL-E. Firstly, VALL-E is a text-to-speech model trained in a language modeling manner with text supervision, while our work focuses on textless generative speech LMs. Secondly, the ICL capability in VALL-E is to learn the acoustic conditions of a given speech segment rather than performing a new task that hasn't been encountered during the pre-training stage. VALL-E consistently performs the text-to-speech task, whereas our work focuses on the typical ICL scenario in an LM and is expected to learn the analogy of the demonstrations.

% \subsection{Prompting Speech Language Models}
% In this paper, we apply prompt tuning to a speech LM to perform warmup training for ICL. This approach is inspired by the recent works~\cite{chang22e_interspeech, wu2023speechgen}, which has demonstrated that prompts can guide the pre-trained speech LM in performing various tasks in an efficient manner.
% SpeechPrompt v2~\cite{chang2023speechprompt} further demonstrates the ability of prompt tuning for transfer learning in a wide range of speech classification tasks.
% Model reprogramming~\cite{DBLP:conf/iclr/ElsayedGS19, DBLP:journals/corr/abs-2202-10629} is another method similar to prompting and can be used for task adaptation. 
% It involves applying a task-specific transformation to the input data, allowing the pre-trained model to adapt to a new task. For example, in~\cite{yen2021neural}, model reprogramming is applied to an acoustic model to adapt it to low-resource spoken command recognition (SCR). And ~\cite{radhakrishnan2023parameter, yang2023english} use reprogramming for domain adaptation in dialect identification and speech recognition.
% Although the aforementioned works can apply prompting or reprogramming methods to adapt a model to new tasks, they do not perform ICL and require further training to adapt to new tasks.
